How to Steer Your Adversary: Targeted and Efficient Model Stealing Defenses with Gradient Redirection

Model stealing attacks present a dilemma for public machine learning APIs. To protect financial investments, companies may be forced to withhold important information about their models that could facilitate theft, including uncertainty estimates and prediction explanations. This compromise is harmful not only to users but also to external transparency. Model stealing defenses seek to resolve this dilemma by making models harder to steal while preserving utility for benign users. However, existing defenses have poor performance in practice, either requiring enormous computational overheads or severe utility trade-offs. To meet these challenges, we present a new approach to model stealing defenses called gradient redirection. At the core of our approach is a provably optimal, efficient algorithm for steering an adversary's training updates in a targeted manner. Combined with improvements to surrogate networks and a novel coordinated defense strategy, our gradient redirection defense, called GRAD${}^2$, achieves small utility trade-offs and low computational overhead, outperforming the best prior defenses. Moreover, we demonstrate how gradient redirection enables reprogramming the adversary with arbitrary behavior, which we hope will foster work on new avenues of defense.

==> comments.tex <==
NOTE: Your setting isn't ``black-box''. It's worse. You don't have query access to the adversary's model. All you have is access to the inputs they are using to train their model.

In the table, have error metrics be "+VAL" instead of just "VAL"



FIGURES & TABLES:
- banner figure like what's on our whiteboard
- pretty curves figure for gradient redirection (we're better than MAD for a fixed budget, even by their own metric; also show the random points for the inner product case)
- banner figure with 3 result plots (CIFAR-10, CIFAR-100, CUB200). For each plot, show the major methods. Also have a second row for calibration.
- small, side table with clean accuracy, unprotected accuracy with both threat models. Rows for CIFAR-10, CIFAR-100, CUB200.
- big table with 19 columns (1 col on left + 3 budgets * 3 datasets * 2 metrics), one row for each method (5 rows)


We want to write down the surrogate's parameters. Give them a symbol.



% \section{Model Stealing Defense}
% We develop a new model stealing defense based on the gradient redirection algorithm in Section \ref{sec:gradient_redirection}. As the adversary's network is unknown to the defender, we cannot directly apply the algorithm. Thus, we represent the adversary with a surrogate network and design optimal perturbations for the surrogate instead.
% % gradient redirection is a general tool; here we describe a model stealing defense

% \subsection{Improving Surrogate Networks}
% Prior work seeking to maximally perturb the adversary's backward pass has explored several different kinds of surrogates, including randomly initialized networks \cite{Orekondy2020PredictionPT} and ensembles of the defender's network at various points throughout training \cite{wallace2020imitation}. However, these works do not analyze the effectiveness of surrogates in detail. Given that our goal is to perturb the adversary's update gradient in a targeted manner, a central question is whether perturbations designed for a surrogate network actually transfer to the adversary.

% \noindent\textbf{Measuring Transfer Performance.}\quad
% cosine distance transfer profile definition
% inner product transfer profile definition
% we use the cifar100->cifar10 setting for these analysis experiments. use symbols from threat model section and briefly describe setup.

% \noindent\textbf{Improving Transfer Performance.}\quad
% We observe that a defender will incrementally be given access to an attacker's query dataset. If the query dataset is of a recognizable type, then the defender can guess what the remaining queries will look like and choose an appropriate surrogate model. This greatly improves transfer.

% \noindent\textbf{Random Surrogates Transfer Poorly.}\quad
% cosine distance profiles for MAD, random perturbation, and ours.

% \noindent\textbf{Stage of Training Affects Transfer.}\quad
% inner product profiles for all-ones vector, stopping after different numbers of epochs. Intuitive result. But which one is better for downstream defense? Does an ensemble work best?

% \subsection{Coordinating Perturbations}
% We use a coordinated defense. Argue that things can cancel out or be less effective. MIN-IP defense is less effective than ALL-ONES, indicating that consistently pushing in an unhelpful direction can be more impactful than maximally pushing away from the clean gradient.

% \subsection{Complete Defense}
% Describe our full defense, derived from our investigation of surrogate networks and coordination.
